HeteroGenManip: Generalizable Manipulation For Heterogeneous Object Interactions

Generalizable manipulation involving cross-type object interactions is a critical yet challenging capability in robotics. To reliably accomplish such tasks, robots must address two fundamental challenges: "where to manipulate" (contact point localization) and "how to manipulate" (subsequent interaction trajectory planning). Existing foundation-model-based approaches often adopt end-to-end learning that obscures the distinction between these stages, exacerbating error accumulation in long-horizon tasks. Furthermore, they typically rely on a single uniform model, which fails to capture the diverse, category-specific features required for heterogeneous objects. To overcome these limitations, we propose HeteroGenManip, a task-conditioned, two-stage framework designed to decouple initial grasp from complex interaction execution. First, Foundation-Correspondence-Guided Grasp module leverages structural priors to align the initial contact state, thereby significantly reducing the pose uncertainty of grasping. Subsequently, Multi-Foundation-Model Diffusion Policy (MFMDP) routes objects to category-specialized foundation models, integrating fine-grained geometric information with highly-variable part features via a dual-stream cross-attention mechanism. Experimental evaluations demonstrate that HeteroGenManip achieves robust intra-category shape and pose generalization. The framework achieves an average 31% performance improvement in simulation tasks with broad type setting, alongside a 36.7% gain across four real-world tasks with different interaction types.

==> tex/Limitations.tex <==
\section{LIMITATION}
\label{limit}
Although our manipulation framework has demonstrated excellent performance across various types of tasks, it still has several limitations. First, the input point clouds we use are all single-view point clouds, so the extraction of object semantic features using these point clouds is highly dependent on the capability of foundation models and camera perspectives. Second, our framework requires object point clouds as input, which necessitates segmenting the target with a 2D vision model first and then projecting it into point cloud; however, the segmentation results and depth map quality for some objects (such as thin-edged hangers and clotheslines) are poor, which severely limits the real-world performance of our framework.
